Pushan: Trace-Free Deobfuscation of Virtualization-Obfuscated Binaries

In the ever-evolving battle against malware, binary obfuscation techniques are a formidable barrier to effective analysis by both human security analysts and automated systems. In particular, virtualization or VM-based obfuscation is one of the strongest protection mechanisms that evade automated analysis. Despite widespread use of virtualization, existing automated deobfuscation techniques suffer from three major drawbacks. First, they only work on execution traces, which prevents them from recovering all logic in an obfuscated binary. Second, they depend on dynamic symbolic execution, which is expensive and does not scale in practice. Third, they cannot generate "well-formed" code, which prevents existing binary decompilers from generating human-friendly output. This paper introduces PUSHAN, a novel and generic technique for deobfuscating virtualization-obfuscated binaries while overcoming the limitations of existing techniques. PUSHAN is trace-free and avoids path-constraint accumulation by using VPC-sensitive, constraint-free symbolic emulation to recover a complete CFG of the virtualized function. It is the first approach that also decompiles the protected code into high-quality C pseudocode to enable effective analysis. Crucially, PUSHAN circumvents reliance on path satisfiability, a known NP-hard problem that hampers scalability. We evaluate PUSHAN on more than 1,000 binaries, including targets protected by academic state of the art (Tigress) and commercial-strength obfuscators VMProtect and Themida. PUSHAN successfully deobfuscates these binaries, retrieves their complete CFGs, and decompiles them to C pseudocode. We further demonstrate applicability by analyzing a previously unanalyzed VMProtect-obfuscated malware sample from VirusTotal, where our decompiled output enables LLM-assisted code simplification, reuse, and program understanding.

==> Makefile <==
DOC = main.tex
PDFLATEX = pdflatex --shell-escape -interaction=nonstopmode -file-line-error
#PDFLATEX = latex2rtf
BIBTEX = bibtex
RERUN = "(There were undefined (references|citations)|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
TARDIR = $(DOC:.tex=-src)
IMG_SRCS = $(wildcard figures/*-source.pdf)
IMG_OBJS = $(patsubst %-source.pdf,%.eps,$(IMG_SRCS))

ALL_TEX_FILES = $(shell find . -type f -name '*.tex')
BIB_FILES = $(wildcard *.bib)

.PHONY: pdf clean

pdf: images $(DOC:.tex=.pdf)

all: pdf

%.pdf: %.tex *.tex $(BIB_FILES) $(IMG_OBJS) $(ALL_TEX_FILES)
	$(eval DOC_BASE := $(GENS)$(shell basename $@ .pdf))
	rm -f $(DOC_BASE).bbl
	${PDFLATEX} $<
	egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(PDFLATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(PDFLATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(PDFLATEX) $<) ; true
	egrep -i "(Reference|Citation).*undefined" $*.log ; true
#	dvips -o $(DOC_BASE).ps -t letter $(DOC_BASE).dvi
#	ps2pdf14 -dPDFSETTINGS=/prepress -dEmbedAllFonts=true $(DOC_BASE).ps


clean:
	find . -name "*.aux" | xargs rm -f
	find . -name "*.log" | xargs rm -f
	find . -name "*.out" | xargs rm -f
	find . -name "*.bbl" | xargs rm -f
	find . -name "*.blg" | xargs rm -f
	@\rm -f \
        $(DOC:.tex=.dvi) \
        $(DOC:.tex=.pdf) \
        $(DOC:.tex=.ps)  \
        $(DOC:.tex=.bbl) \
        $(DOC:.tex=.blg) \
        $(DOC:.tex=.lof) \
        $(DOC:.tex=.lot) \
        $(DOC:.tex=.loc) \
        $(DOC:.tex=.lol) \
	$(DOC:.tex=-src.tar.gz)

watch:
	make; fswatch -0 `find . -name "*.tex" -o -name "*.bib"` | xargs -0 -n1 make all

images: $(IMG_OBJS)

%.eps: %-source.pdf
	pdftops -eps $< $(<:-source.pdf=.eps)

veryclean: clean
	@\rm -f *~ *.log
	@\rm -f figures/*.eps

tar: pdf
	@test -d $(TARDIR) || mkdir $(TARDIR)
	@cp Makefile *.{tex,bib,bst,cls} $(TARDIR)
	@tar cz $(TARDIR) > $(TARDIR).tar.gz
	@rm -rf $(TARDIR)


==> old/arch.tex <==
%-------------------------------------------------------------------------------
\section{Fraudulent E-Commerce Website \\Classification}
\label{s:method}
%-------------------------------------------------------------------------------



==> old/data.tex <==
%-------------------------------------------------------------------------------
\section{Data Collection, Validation, and Analysis}




==> old/furtheranalysis.tex <==
%-------------------------------------------------------------------------------
\section{Further Analysis}
\label{s:further}
%-------------------------------------------------------------------------------

\subsection{User Study}
Talk about the bot experiment

\subsection{Scam Websites Characteristics}
Talking about the common characteristics of scam websites including a timeline and how they are changing over time.


==> old/goal-and-scope.tex <==
\section{Goal and Scope}


==> old/implementation.tex <==
%\section{Implementation}
%We implemented our pipeline on top of angr, an open-source binary analysis framework.
%To implement the CFG Recovery, we modified a version of angr's CFGEmulated class to handle data-sensitive basic blocks.



==> reviews/sp_diffsummary.tex <==
\onecolumn
\thispagestyle{empty}

\noindent \textsc{\large Summary of Changes}
\vspace{5pt}

\noindent We thank all the reviewers for their careful reviews and constructive suggestions.
In the revision, we address the concerns to the best of our ability. Please find our responses to the requested changes as follows.

\begin{enumerate}

\item  \emph{Detailed discussion and evaluation of the robustness of the features. Only verbal discussion is not
adequate, the reviewers expect to see a thorough evaluation. In case, the features are found to be
not robust, redesigning some of the features (social network links related ones) is expected}.

We conducted a comprehensive analysis to evaluate the robustness of our designed features using feature perturbation in \hyperref[diff:robust]{Section~\ref{diff:robust}}.
For each class of features, we discuss what specific features an adversary can alter, and, when appropriate, we calculate financial costs that the adversary needs to pay for changing such features.
For instance, domain age is a feature that we use in the proposed classifier.
Hence, an adversary can purchase an old domain to evade detection.
We included an analysis of the success rate along with the cost of acquiring such aged domain names.
Our analysis results show that, although the miscreants can deceive the classifier by altering several features, such efforts would be cost-prohibitive for them.
% will be very high.


\item \emph{Provide a clear problem definition.
What is in scope and what is not?
How did you determine that?}

Based on the collected data, we narrow down the problem definition to detecting malicious shopping, charity, and petscam websites.
These three categories cover more than 70\% of our dataset.
%  which is based on real-world information that has been published on Reddit.
We define the scope of the problem in \hyperref[diff:probdef]{Section~\ref{diff:probdef}}.
Further, to show the extensibility of the proposed method, we evaluated our classifier (trained on the these three categories) on the rest of the scam websites in \hyperref[diff:extend]{Section~\ref{diff:extend}}.

\item \emph{More detailed discussion and comparison with relevant previous work.}

% To improve the experiments,
% We added a low false positive variant of our proposed model as a new baseline.
%Cantina+ is a powerful and well-known phishing detection model.
% We train and test the Cantina+ model on our dataset.
% similar to the proposed model.
% The comparison results are in \hyperref[diff:baselines]{Section~\ref{diff:baselines}}.
We added [1, 2] to our related work and planned to include them as baselines suggested by the reviewers.
However, unfortunately, the source code and data of the models are not publicly available.
Therefore, we sent repeated emails to all authors of the suggested papers over the course of several months asking for access to the course code and data.
Authors of [1] responded to our request to tell us that unfortunately they no longer have access to the data and code.
The Surveylance~[2] authors responded to our request, but unfortunately we only received partial code and data, which were not usable to reproduce their results.

However, we extended our evaluation and compared against Cantina+, which a powerful and well-known phishing detection model.
The comparison results are in \hyperref[diff:baselines]{Section~\ref{diff:baselines}}.


% We discussed regarding this circumstance in \hyperref[diff:metrics]{Section~\ref{diff:metrics}}.
% The information can be found in \hyperref[diff:metrics]{Section~\ref{diff:metrics}}.

\item \emph{Improved discussion of the quality of labels and the possibility of using multiple labeling sources.}

We improved the data labeling process in \hyperref[diff:labeling]{Section~\ref{diff:labeling}} as follows: We changed our labeling function based on the number of positive and negative comments in response to URLs.
Moreover, we use ScamAdviser as a secondary source of labeling to verify the quality of our labeling process.
We leverage ScamAdviser's API to receive legitimacy labels of our collected URLs.
We added the information in \hyperref[diff:labelvalid]{Section~\ref{diff:labelvalid}}.
% However, according to our manual analysis, ScamAdviser seems to have a high false negative rate.
% Therefore, we only changed the labels of legitimate URLs to a scam if they are detected as malicious ones by ScamAdviser.
%

\item \emph{More fair discussion of and comparison with content-based detectors and URL blocklists}:

For better comparison and evaluation, we evaluated another content-based detector, Cantina+ in \hyperref[diff:baselines]{Section~\ref{diff:baselines}}.
To have a fair comparison we use our dataset to train and test the Cantina+ model.
Moreover, we did not use URL blocklists for comparison purpose.
By providing blocklists results on our dataset, we aim to reveal current ecosystems' lack of defense against non-phishing scam websites.

\item \emph{Better presentation of the experimental results.
Especially, a better evaluation of false positives and detailed FP analysis with case studies.
Also, better highlight the TPR obtained at low FPR (since the classifier would not be usable at high FPRs).
Here we do not only expect the FP evaluation with benign websites but also with other types of malicious websites.
It is important to understand how specific designed features are for the non-phishing scam sites the authors aim at detecting:}

To better illustrate the effectiveness of our proposed model, we added evaluation metrics in Table~\ref{tab:performance} and Table~\ref{tab:performance_ext}.
We also added two more baselines, Cantina+ and a low false positive variant of the proposed model.
Moreover, we applied our model to the bottom 10K of the top Alexa 1M websites to evaluate the effectiveness of the proposed classifier.
The evaluation results are in \hyperref[diff:alexa]{Section~\ref{diff:alexa}}, which shows that our method has a low false positive rate with high accuracy.

To show the uniqueness of the designed features, we extent our experiments to evaluate the proposed model on the malware and defacement websites in \hyperref[diff:othermalicious]{Section~\ref{diff:othermalicious}}.
The results indicate that the proposed model is not suitable to detect such websites as the features are designed for detecting scam websites.

\item Other changes that we made based on the reviews:

        \begin{enumerate}
            \item [a.] We discussed more papers related to our work in \hyperref[diff:relwork]{Section~\ref{diff:relwork}}.
            \item [b.] To increase the stability and the performance of the proposed model, we added social media-based features that gives us an additional insight about the legitimacy of a website.
              Information regarding these novel features can be found in \hyperref[diff:smf]{Section~\ref{diff:smf}}.
            \item [c.] We expanded \hyperref[diff:labelvalid]{Section~\ref{diff:labelvalid}} to discuss how we validate labels through human experts.
            % include details on validating labels manually by human experts, one author and two non-authors.
        \end{enumerate}
\end{enumerate}
\label{diff:probdef} % put this at location of diff

\noindent\textsc{\large Summary of Changes References}

{\small
\noindent [1] Srinivasan, B., Kountouras, A., Miramirkhani, N., Alam, M., Nikiforakis, N., Antonakakis, M., \& Ahamad, M. (2018, April). Exposing search and advertisement abuse tactics and infrastructure of technical support scammers. In Proceedings of the 2018 World Wide Web Conference (pp. 319-328).

\noindent [2] Kharraz, A., Robertson, W., \& Kirda, E. (2018, May). Surveylance: automatically detecting online survey scams. In 2018 IEEE Symposium on Security and Privacy (SP) (pp. 70-86). IEEE.
}

% reset everything as if this page didn't exist
\twocolumn
\clearpage
\pagenumbering{arabic}





% Improve the discussion of how scam websites can be reviewed and identified as such.

% Focus more on demonstrating how to create a great dataset, including demonstrating the
% improvement in dataset quality in the evaluation. There have been lots of papers on how to do
% phishing detection, and it isn't immediately clear that those techniques wouldn't apply to these
% sites as well (and it's OK if they do) but then the contribution here has to be more around how to
% produce a dataset and demonstrating that the detector works.

% Focus more on an evaluation demonstrating real-world impact (e.g. finding loads of new scam
% websites with high precision)

% Looking at payment features as part of the analysis would be cool to see.

% A new classifier with a set of features that address the dynamic nature of the problem and go
% deeper into accounting for the real-world adversary.

% A better labeling method for the scam sites (relying on a custom classifier for the scam settings)

% A discussion of the evasion mechanisms and how they can be avoided.

% Designing the solution while accounting for the real world scenario of highly imbalanced data.
% Discussing the implications of such a setting on the deployment.

% Better problem definition.

% Better discussion and comparison with relevant previous work.

% Better discussion of quality of labels and use of multiple labeling sources, whenever possible.

% Discussion and evaluation of the robustness of the features.

% Better presentation of the experimental results (highlight TPR at low FPR, for instance by using a
% better ROC analysis and partial AUC).

% More fair discussion of and comparison with content-based detectors and URL blocklists.


==> scam_types.tex <==
\section{Non-phishing Scam Categories}
\label{ss:scam_types}
In this section we categorize different types of non-phishing scam websites according to their content. 
For the sake of simplicity we use the term ``scam websites'' to refer to non-phishing scam websites.
We analyzed the source code of our collected data (\autoref{s:collection}) to assign each website to a category using keywords:

\begin{itemize}
    \item \textbf{Fraudulent Online Shopping Website.} Fraudulent online shopping websites are the most common among malicious websites. These websites try to keep up with the legitimate websites in order to lure users. Miscreants try to create a shopping website similar to legitimate websites having rare or discounted items. Rare items make these website more visible to users while they try to search for them, while discounted items attracts more visitors. Specifically, they use different techniques such as limited time offers or showing recent purchases as notifications in order to rush users into buying the items~\cite{bitaab2020scampandamic}. 

    \item \textbf{Pet scams.} Pet scams are malicious websites claims to sell pets at a cheaper price than market. Miscreants aim to get victims emotionally attached to fictitious pet. These kinds of websites appear to be legitimate at first glance since most of them do not have any on-site payment option. Rather, the miscreants ask users fill out an application to be reviewed for eligibility. The designed process of buying pets makes the users even more attached to the fictitious pet and it will become easier for the criminals to extort money from users. Moreover, in most cases, they use a fraudulent shipping website in order to lengthen the process~\cite{ecrime_petscam}.
    
    \item \textbf{Charity Websites.} These websites mainly leverage real world scenarios in order to take advantage of users empathy. Fake charity or donation websites lure users into thinking that they are helping people in need, while they are stealing information or getting non-refundable money. As an example, during the recent COVID-19 pandemic, the attackers used this event in order to create fake charity website, using people's emotion in order to gather both money and information.
    
    \item \textbf{Cryptocurrency.} People consider cryptocurrency as a stable investment~\cite{mnif2020cryptocurrency}. This creates an opportunity for the social engineering attackers to lure internet users into investing on their malicious cryptocurrency websites.
    \item \textbf{Stock Market.} Malicious stock market websites follow a similar approach to fake cryptocurrency. Most of them lure users into investing in stocks by showing high interest stocks from non-existing companies. 
    
    \item \textbf{Education Related Websites.} These malicious websites mostly target students who need help in writing essays, research papers, and other types of homeworks. In some of these websites, miscreants get information from students and make them pay a specific amount of money in exchange for not getting reported to their school~\cite{bbbextortion}.
    
    \item \textbf{Delivery Websites.} Malicious delivery websites act as a support website for social engineering attackers who want to sell items to users. They can be used in the pet scam and fake online shopping websites to show a fake path and tracking for a non-existing package. The delivery websites can cause the aforementioned websites live longer as they can show a delay in the sent packages, making the users believe that the problem is the shipping company. 
    
    \item \textbf{Adult Content.} This category includes websites related to adult content such as dating websites.
    
    \item \textbf{Business Related Websites.} Banking websites and websites encouraging users to make investments for high yield profits are considered as business related websites.
    
    \item \textbf{Other.} This category includes other types of websites such as adult content, tech support scams, and credit services.
\end{itemize}
